A Near-Optimal Sublinear-Time Algorithm for Approximating the Minimum Vertex Cover Size

We give a nearly optimal sublinear-time algorithm for approximating the size of a minimum vertex cover in a graph G. The algorithm may query the degree deg(v) of any vertex v of its choice, and for each 1 <= i <= deg(v), it may ask for the i-th neighbor of v. Letting VC_opt(G) denote the minimum size of vertex cover in G, the algorithm outputs, with high constant success probability, an estimate VC_estimate(G) such that VC_opt(G) <= VC_estimate(G) <= 2 * VC_opt(G) + epsilon*n, where epsilon is a given additive approximation parameter. We refer to such an estimate as a (2,epsilon)-estimate. The query complexity and running time of the algorithm are ~O(avg_deg * poly(1/epsilon)), where avg_deg denotes the average vertex degree in the graph. The best previously known sublinear algorithm, of Yoshida et al. (STOC 2009), has query complexity and running time O(d^4/epsilon^2), where d is the maximum degree in the graph. Given the lower bound of Omega(avg_deg) (for constant epsilon) for obtaining such an estimate (with any constant multiplicative factor) due to Parnas and Ron (TCS 2007), our result is nearly optimal. In the case that the graph is dense, that is, the number of edges is Theta(n^2), we consider another model, in which the algorithm may ask, for any pair of vertices u and v, whether there is an edge between u and v. We show how to adapt the algorithm that uses neighbor queries to this model and obtain an algorithm that outputs a (2,epsilon)-estimate of the size of a minimum vertex cover whose query complexity and running time are ~O(n) * poly(1/epsilon).

==> averageDegree.tex <==
\section{Average Degree $\hat{d}$}
\label{averageDegree.sec}

Our analysis considers $d$ as the maximum degree. We shall show the same bounds for average degree.\\
Denote $\hat{d}$ as the average degree in the graph.
Consider a high degree vertex as a vertex with degree $>\frac{4\hat{d}}{\eps}$. Denote $H$ the group of all high vertices in $G$. Denote $G' = (V \setminus H, E')$ where $E'\subseteq E$ are all edges in $G$ that adjacent to a vertex in $H$.
We will modify $VO^\pi$ and $MO^\pi$ as follows:
If $v\in H$, i.e. has degree $>\frac{4\hat{d}}{\eps}$ then $VO^\pi(v)$ will return TRUE. Otherwise it will run as before, calling $MO^\pi$ on graph $G'$.
$|\VC_{opt}| \leq |\VC^\pi(G)| \leq |H| + |\VC^\pi(G')| \leq 2|\VC_{opt}| + \frac{\eps n }{4}$.
\mnote{M: need to explain more and also show that it works fine with mm part}.

==> dense.tex <==
\subsection{Adapting the Algorithm to Dense Graphs}\label{dense.sec}

The focus of this paper was on designing a sublinear algorithm whose access to
the graph  is via degree queries and neighbor queries. In other words, we assumed
that the graph was represented by adjacency lists (of known lengths).
When a graph is dense (i.e., when the number of edges is $\Theta(n^2)$),
then a natural alternative representation is by an adjacency matrix.
This representation supports queries of the form: ``Is there an edge between
vertex $u$ and vertex $v$?'', which we refer to as {\em vertex-pair\/} queries.

We next show how to adapt the algorithm described in the previous section 
to an algorithm that performs vertex-pair queries. 
The query complexity and running time of the algorithm are (with high constant
probability) $\tilde{O}(n/\eps^4)$, which is linear in the average degree for
dense graphs. As in the previous section, the algorithm outputs
(with high constant probability)
a $(2,\eps)$-estimate of the size of the minimum vertex cover.
We recall that the linear lower bound in the average degree~\cite{PR} 
also holds for the case that the average degree is $\Theta(n)$ and 
when vertex-pair queries are allowed.

Given a graph $G = (V,E)$, let $\tG = (\tV,\tE)$ be a supergraph of $G$ that is
defined as follows. For every vertex $v \in V$ whose degree in $G$ is less than\footnote{
If there are no self-loops in the original graph, then the bound is $n-1$.} $n$,
there exists a vertex $v' \in \tV$, where there are $\deg_G(v) - n$ parallel
edges between $v$ and $v'$, and there are $(8/\eps)n$ self-loops incident to $v'$.
As shown in Subsection~\ref{var-deg.subsec}, with high probability over the choice
of a ranking $\tilde{\pi}$ over $\tG$, we have that 
$|\VC^{\tilde{\pi}}(\tG) \cap V| \leq 2 |\VCopt(G)| + (\eps/4)n$. 

Note that we can emulate neighbor queries to $\tG$ given access to vertex-pair
queries in $G$ as follows. Let the vertices in $G$ be $\{1,\ldots,n\}$. When 
the $j^{\rm th}$ neighbor of vertex $i$ is queried, then the answer to the
query is $j$ when $(i,j) \in E$, and it is $i'$ (the new auxiliary vertex adjacent
to $i$) when $(i,j) \notin E$. The degree of every vertex in $V$ is $n$, so there
is no need to perform degree queries.
Since the ratio between the maximum degree and the minimum degree in
$\tG$ is at most $1/\eps$, and the maximum and average degrees are $O(n/\eps)$,
we obtain an algorithm whose complexity is $\tilde{O}(n/\eps^4)$, as claimed.


==> lb.tex <==
\section{A Lower Bound for Finding an Approximately Minimum Vertex Cover}
A natural question is whether there is an algorithm whose complexity
is sublinear in the size of the graph for {\em finding\/} 
a vertex cover whose size is at most $ \alpha \cdot |\VCopt(G)| + \eps n$
for some $\alpha \geq 1$ and $\eps < 1$ (recall that $\VCopt(G)$ denotes 
a minimum vertex cover for $G$). Here we answer this question
negatively (where our lower bound construction is somewhat similar to
the one presented in~\cite{PR} for approximating the size of the
minimum vertex cover). 

Specifically, we say that an algorithm is an $(\alpha,\eps)$-approximation
algorithm for the minimum vertex cover for a fixed constant $\alpha>1$, if, 
given query access to any graph $G$ and a parameter $\epsilon <1$,
with probability at least $2/3$ the algorithm outputs a set $C$ such that $C$ is a vertex
cover for $G$ and $|C| \leq |\VCopt(G)| + \eps n$.
\BT
\label{lb-gen.thm}
For any $n$, $\alpha> 1$, and $\hat{m} \leq \ldots $, % \frac{n(n-1)}{4\alpha}$,
every $(\alpha,\eps)$-approximation algorithm for the minimum vertex cover
of graphs with $\Theta(\hat{m})$ requires $\Omega(m)$ queries. This lower bound holds
when all types of queries are allowed (i.e., neighbor queries, degree queries and
vertex-pair queries).
\ET

\BPF
We first prove the theorem for $\hat{m} =\Theta(n^2)$ and for 
$\alpha =2$. We later explain how to modify it to the case of sparser
graphs and larger $\alpha$.
Consider the family of graphs that are 
all slightly modified versions of the complete bipartite graph $K_{n/4,3n/4}$.
Let $L$ denote the set of $n/4$ vertices on the left hand side
of $K_{n/4,3n/4}$, and let $R$ denote the $3n/4$ vertices on the right hand side.
Each graph in the family is determined by selecting a pair of vertices
$u_L,v_L \in L$ and a pair of vertices $u_R,v_R \in R$, removing the
edges $(u_L,u_R)$ and $(v_L,v_R)$, and adding the edges
$(u_L,v_L)$ and $(u_R,v_R)$.
We also allow all possible labelings of the edges incident to each vertex,
but assume that the vertices in $L$ are labeled $1,\ldots,n/4$, while
the vertices in $R$ are labeled $n/4+1,\ldots,n$.
 Let the resulting family of graphs be denoted ${\cal G}$.

First note that for each graph in ${\cal G}$ there is a minimum vertex cover
of size $n/4 + 1$, which consists of $L$ and either $u_R$ or $v_R$.
The intuition is that for a uniformly selected graph in
${\cal G}$, if the algorithm performs at most $m/c$ queries for some
sufficiently large constant $c$, then it will not be able to determine
the identity of $u_R$ or $v_R$. Since it must output a set of size
at most $2(n/4+1) + \eps n$, for any $\eps < 1/8$, it will not be able
to ``hit'' any of the two vertices. We next formalize this argument.

We consider a process that interacts with any algorithm for finding
an approximately minimum vertex cover and answers
the algorithm's queries while constructing a uniformly selected graph in
${\cal G}$.  Since all vertices in $L$ have degree $3n/4$ and all vertices in
$R$ have degree $n/4$, and since for each vertex it is known whether it is
in $L$ or in $R$, we may assume without loss of generality that the algorithm
does not ask any degree queries.
At the start of each step $t$ of the algorithm there is the current {\em knowledge graph}, 
denoted $K_t$,
which consists of those edges (and ``non-edges'') that the algorithm
revealed in its (neighbor and vertex-pair) queries. 
Once the algorithm terminates, the process completes
the construction of the uniformly selected graph. 

The information concerning known edges in
the knowledge graph can be represented by two tables: $T_L$ and $T_R$,
where in $T_L$ there is a row for each vertex in $L$ and in $T_R$ there is
a row for each vertex in $T_R$. In $T_L$ there are $3n/4$ columns, where
for $v \in L$ the entry $T_L[v,i]$ is simply the $i^{\rm th}$ neighbor of
vertex $v$, and in $T_R$ there are similarly $n/4$ columns. Observe that
for each vertex $w \in L$ except for $u_L$ and $v_L$, the row $T_L[w,\cdot]$
is simply a permutation of the vertices in $R$, and an anlogous statement
holds for $w \in R$ such that $w \notin \{u_R,v_R\}$.  
We assume for simplicity that
if the algorithm asks a vertex-pair query $(u,v)$ and gets a positive answer,
then it also gets the labels of the edge according to its two endpoints
(that is, it gets the two corresponding entries in the table(s)).
Similarly, if it asks a neighbor query $(w,i)$ and gets as an answer a vertex
$z$, then it also gets the label $j$ of the edge $(w,z)$ in the list of edges
incident to $z$.
In addition, the knowlege graph contains information concerning negative
answers to vertex-pair queries.
We may assume without loss of generality that the algorithm does not ask queries
whose answer is contained in the knowledge graph.

If at any point the knowledge graph either contains an edge between two vertices
in $L$ or between two vertices in $R$, or it contains a non-edge between a
vertex in $L$ and a vertex in $R$, then we may assume that the algorithm
terminates with a minimum vertex cover (possibly after asking $O(n)$ additional queries in case 
it found an edge between two vertices in $L$). Otherwise,
given a new query $q_t$, the process answers it as follows.
Let $m_t$ denote the number of edges in the knoweldge graph $K_t$ (where all these edges
are between vertices in $L$ and vertices in $R$), and let $\bar{m}_t(L)$ 
denote the number of non-edges between pairs of vertics in $L$
in the knoweldge graph $K_t$, and similarly define $\bar{m}_t(R)$. 
Observe that $m_t+\bar{m}_t(L)+\bar{m}_t(R) \leq t-1$.
For a vertex
$v$ let $\Gamma_t(v)$ denote the set of neighbors that $v$ has in $K_t$ and
let $\bar{\Gamma}_t(v)$ denote the set of its ``non-neighbors'' (that is, $u$
such that the vertex-pair query $(u,v)$ was answered negatively).
% Let $m_t(v) = |\Gamma_t(v)|$ and $\bar{m}_t(v) = |\bar{\Gamma}_t(v)|$.
\BE
\item If $q_t$ is a vertex-pair query, $(w,z)$, where $w \in L$ and $z \in R$,
then the algorithm gives a negative answer with probability  that is upper bounded by
$\frac{2}{3n^2/16 - m_t}$ (this is an upper bound since if $(w,x)$ is a non-edge
in $K_t$ for every $x \in L$ or $(z,y)$ is a non-edge for every non-edge in $K_t$,
then this probability is $0$).
% (which for $t \leq n^2/c$ and a sufficiently large constant $c$,
% is $O(1/n^2)$). 
If the answer is positive, then the process uniformly selects an empty
entry in $T_L[w,\cdot]$ and an empty entry in $T_R[z,\cdot]$, and fills them with
$z$ and $w$, respectively. 
\item If $q_t$ is a vertex-pair query, $(w,z)$, where $w,z \in L$, then the
algorithm gives a positive answer with probability that is upper bounded by
$\frac{1}{(n/4)(n/4-1)/2 - \bar{m}_t(L)}$. Similarly, if  $w,z \in R$, then the
algorithm gives a positive answer with probability that is upper bounded by
$\frac{1}{(3n/4)(3n/4-1)/2 -  \bar{m}_t(R)}$.
\item If $q_t$ is a neighbor query, $(w,i)$ where $w \in L$, then the process
first flips a coin with bias that is
upper bounded
\mnote{D: I am not completely sure about this}
 by $\frac{2}{3n^2/16 - (m_t + \bar{m}_t(L))}$ to decide whether
the answer is a vertex in $L$. If not, then it uniformly selects a vertex 
$z\in R\setminus \Gamma_t(w)$ (and sets $T_L[w,i]=z$ and $T_R[z,j] = w$ for
a uniformly selected empty column $j$ in $z$'s row in $T_R$). If the answer
is determined to be in $L$, then the process uniformly selects an empty entry
$T_L[z,j]$ (where $(w,z)$ is not a non-edge in $K_t$), and answers accordingly.
\EE
By the above, if the algorithm performs at most $n^2/c$ queries
and a sufficiently large constant $c$,
 then the probability that it either detects a non-edge
between a vertex in $L$ and a vertex in $R$, or it detects an edge between
two vertices in $L$ or two vertices in $R$ in any query, is a small constant.
Assuming such an event did not occur, let $C$ be set of vertices that the
algorithm outputs, where $|C| \leq n/2 + 2 +\eps n$, which for $\eps < 1/8$ is
at most $17n/8 + 2$. 
\EPF




==> var-deg.tex <==
\section{The Near-Optimal Algorithms}

Theorem~\ref{avg-calls.thm} gives a bound on the expected number of recursive calls to oracles,
necessary to compute an answer when the vertex cover oracle is called for a random vertex.
The expected number of calls is $O(\rho\cdot \bd)$,
where $\rho$ is the ratio between
the maximum degree $d$ and the minimum degree $d_{\min}$, and $\bd$ is the 
average degree.

(Recall that we assume without loss of generality that $d_{\min} \geq 1$.
For isolated vertices, the oracle answers that they are not in the vertex cover
in $O(1)$ time, and therefore, it suffices to focus on the subgraph consisting of non-isolated vertices.)

A straightforward application of Theorem~\ref{avg-calls.thm} gives a bound of $O(d^2)$ for graphs with maximum degree bounded by $d$. We show a bound of $O(d/\eps)$ for a \emph{modified} graph, which is preferable if $1/\eps < d$, and we also show how to use the modified graph to obtain an estimate for the minimum vertex cover size in the original input graph. We combine the obtained bound with Lemma~\ref{lem:running_time} to get a fast and query-efficient algorithm.

Next we show how to obtain an efficient algorithm for the case when only the average degree
of the input graph is bounded. Finally, we show how to adapt the algorithm to the dense graph case, when only vertex-pair queries are allowed.


\subsection{Bounded Maximum Degree}

As we have mentioned above, we can assume that $1/\eps < d$.
For a given graph $G = (V,E)$ with maximum degree $d$, 
consider a graph $\tG = (\tV,\tE)$,
such that $\tV = V \cup V'$ and $\tE = E\cup E'$
where $V'$ and $E'$ are defined as follows.
For every vertex $v\in V$, $V'$ contains $v'$,
and $E'$ contains $\lfloor \eps d \rfloor$ parallel edges between 
$v$ and $v'$, and $8d$ parallel self-loops for $v'$.

For a random ranking $\tilde{\pi}$ over $\tE$, 
we are interested in bounding $|\VC^{\tilde{\pi}}(\tG) \cap V|$
as compared to $|\VCopt(G)|$ (the size of a minimum vertex cover of $G$).
Since $\VC^{\tilde{\pi}}(\tG) \cap V$ is a vertex cover of $G$,
we have that $|\VC^{\tilde{\pi}}(\tG) \cap V| \geq |\VCopt(G)| $,
and so we turn to an upper bound on $|\VC^{\tilde{\pi}}(\tG) \cap V|$.

Let $\tilde F$ be the set of all parallel edges connecting each $v$ with the corresponding $v'$.
We have 
$$|\VC^{\tilde{\pi}}(\tG) \cap V| 
    \leq 2|\MM^{\tilde{\pi}}(\tG) \cap E| + |\MM^{\tilde{\pi}}(\tG) \cap \tilde F|
\le 2 |\VCopt(G)| + |\MM^{\tilde{\pi}}(\tG) \cap \tilde F|.$$
Consider an arbitrary ranking $\tilde\pi$ of $\tilde E$.
Observe that for each $v\in V$, the matching
$\MM^{\tilde{\pi}}(\tG)$ either includes a parallel edge between
$v$ and $v'$ or
it includes a self-loop incident to $v'$.
For every $v' \in V'$, if the lowest rank of self-loops incident to $v'$
is lower than the lowest rank of edges $(v,v')$, then
$\MM^{\tilde{\pi}}(\tG)$ contains one of the self-loops, but does not contain
any parallel edge $(v,v')$. If the ranking $\tilde \pi$ is selected uniformly
at random, the above inequality holds independently for each vertex with probability
at least $\eps d / 8 d = \eps/8$. Therefore, the expected number of edges
in $\MM^{\tilde{\pi}}(\tG) \cap \tilde F$ is bounded by
$\eps n/8$. Without loss of generality, we can assume that $\eps n > 72$, since otherwise
we can read the entire input with only $O(1/\eps^2)$ queries and compute a maximal matching in it. It follows from the Chernoff bound that with probability $1-1/20$, $|\MM^{\tilde{\pi}}(\tG) \cap \tilde F| \le \eps n/4$.


Observe that given query access to $G$, we can provide query access to $\tG$
(in particular, the edges in $E'$ that are incident to each $v\in S$ can be indexed starting
from $\deg(v)+1$). Every query to $\tG$ can be answered in $O(1)$ time, using $O(1)$
queries to $G$. Therefore, we can simulate an execution of the vertex-cover and the maximal-matching oracles on $\tG$.

Note that the expected number of recursive calls to the maximal matching oracle is bounded for a random vertex $v \in \tilde V$ by $O(d/\eps)$, because the maximum degree and the minimum degree are within a factor of $O(1/\eps)$. Note that since $|V| = |\tilde V|/2$, this expectation for a random vertex $v \in V$ is at most twice as much, i.e., it is still $O(d/\eps)$.

For any ranking $\tilde \pi$ of edges in $\tE$,
if we sample $O(1/\eps^2)$ vertices from $V$ with replacement, then the fraction of those in 
$\VC^{\tilde{\pi}}(\tG) \cap V$ is within an additive $\eps / 8$ of $|\VC^{\tilde{\pi}}(\tG) \cap V
| / |V|$ with probability $1 - 1/20$. Let $\mu$ be this fraction of vertices. Applying the union bound, we have 
$$|\VCopt(G)| - \eps n/4 \le \mu \cdot n \le 2 |\VCopt(G)| + \eps n/2$$
with probability $1-1/10$. Then $(\mu + \eps/4) \cdot n$ is the desired $(2,\eps n)$-estimate.
The expected number of calls to the vertex cover and maximal matching oracles is bounded by $O(d/\eps^3)$.  Note that without loss of generality, $\eps \ge 1/4n$,
because any additive approximation to within an additive factor smaller than $1/4$
yields in fact the exact value. Therefore the expected number of calls to the oracles
is bounded by $O(n^4)$, which can be represented with a constant number of machine words in the standard binary representation, using the usual assumption that we can address all vertices of the input graph. By applying now Lemma \ref{lem:running_time},
we obtain an implementation of the algorithm. 
It runs in $O(d/\eps^3 \cdot \log^3(d/\eps))$ time and makes $O(d/\eps^3 \cdot \log^2(d/\eps))$ queries. Moreover, the probability that the implementation diverges from the ideal algorithm is bounded by $1/5$. Therefore, the implementation outputs a $(2,\eps n)$-estimate with probability 
$1 - 1/10 - 1/5 \ge 2/3$.

\begin{corollary}
There is an algorithm in the adjacency list model that runs in $O(\frac{d}{\eps^3} \cdot \log^3\frac{d}{\eps})$ time, makes $O(\frac{d}{\eps^3} \cdot \log^3\frac{d}{\eps})$ queries,
and with probability $2/3$, outputs a  $(2,\eps n)$-estimate to the minimum vertex cover size.
\end{corollary}

\subsection{Bounded Average Degree}

In this section, we assume an upper bound $\bd$ on the average graph degree and show an efficient algorithm in this case. 

Given a graph $G=(V,E)$ with average degree $\bd$,
let $L$ denote the subset of vertices in $G$ whose degree is greater than $8\bd/\eps$.
Hence, $|L| \le \eps n/8$.
Let $E(L)$ denote the subset of edges in $G$ that
are incident to vertices in $L$, and let $\bG = (\bV,\bE)$ be defined by
$\bV = V\setminus L$ and $\bE = E\setminus E(L)$, so that the maximum degree in 
$\bG$ is at most $8\bd/\eps$.
For any maximal matching $\bM$  in $\bG$ we have that
\BEQ
|\VCopt(G)| \leq 2|\bM| + |L| \leq 2|\VCopt(G)| + \frac{\eps}{8}n\;.
\EEQ
Thus, the first modification we make to the oracles
is that if the vertex-cover oracle is 
called on a vertex $v$ such that the degree of $v$ is greater
than $(4/\eps)\bd$, then it immediately returns {\sc true}.\footnote{As shown in~\cite{PR}, 
we don't actually need to know $\bd$ for this
purpose, but it suffices to get a bound that is not much higher than $(4/\eps)\bd$,
and such that the number of vertices with a larger degree is $O(\eps n)$, where such a bound
can be obtained efficiently.} 


We now create a graph $\tG = (\bV \cup \tV,\bE \cup \tE)$ as follows.
For every $v \in \bV$, we add to $\tV$ a vertex $v'$ and vertices $v''_i$, where $1 \le i \le \lceil\deg_G(v)/\bd\rceil$ and $\deg_G(v)$ is the degree of $v$ in $G$. Each of these new vertices has $32\bd/\eps$ parallel self-loops.
Moreover, we add $\bd$ parallel edges between $v$ and $v'$. Finally, partition the edges incident
to $v$ in $G$ into $\lceil\deg_G(v)/\bd\rceil$ groups, each of size at most $\bd$. The first group corresponds has the first $\bd$ edges on the neighborhood list of $v$, the second group corresponds to the next $\bd$ edges, and so on. Let $E_{v,i} \subset E$ be the set of edges in the $i$-th group.
For every $i$ of interest, we add $|E_{v,i} \cap E(L)|$ parallel edges between $v$ and $v''_i$
and $|E_{v,i} \setminus E(L)|$ parallel self-loops incident to $v''_i$. We add these edges so that we are later able to simulate every query to $\tG$ using a constant number of queries to $G$.

Let us bound the total number of vertices in $\tV$. The number of vertices $v'$ is $|\bV|$.
The number of vertices $v''_{i}$ is bounded by 
$$\sum_{v \in \bV} \left\lceil \frac{\deg_G(v)}{\bd} \right\rceil
\le 
\sum_{v \in \bV} \left(\frac{\deg_G(v)}{\bd} + 1\right)
\le 
\frac{\bd \cdot |\bV|}{\bd} + |\bV| = 2 |\bV|,
$$ 
because $\tV$ has been created by removing vertices with highest degrees in $G$,
and the average degree of vertices in $\tV$ in $G$ cannot be greater than $\bd$,
the initial average degree. This shows that $|\tV| \le 3|\bV|$.

We now repeat an argument from the previous section that despite the additional edges and vertices,
$|\VC^{\tilde{\pi}}(\tG) \cap \tV|$ is likely to be a good approximation to $|\VCopt(\bG)|$
for a random ranking $\tilde{\pi}$. First, $\VC^{\tilde{\pi}}(\tG) \cap \tV$ is still a vertex cover for $\bG$, so $|\VCopt(\bG)| \le |\VC^{\tilde{\pi}}(\tG) \cap \tV|$. Let $\tilde F$ be the set of edges connecting all $v$ with the corresponding $v'$ and $v''_i$. 
We have 
$$|\VC^{\tilde{\pi}}(\tG) \cap \bV| 
    \leq 2|\MM^{\tilde{\pi}}(\tG) \cap \bE| + |\MM^{\tilde{\pi}}(\tG) \cap \tilde F|
\le 2 |\VCopt(\bG)| + |\MM^{\tilde{\pi}}(\tG) \cap \tilde F|.$$
Observe that if for some of the vertices in $\tV$, the lowest rank of self-loops is lower than the lowest rank of the parallel edges connecting this vertex to the corresponding vertex in $\bV$, then 
one of the self-loops is selected for the maximal matching as opposed to the parallel edges.
The inequality on ranks does not hold with probability at most $\bd/(32\bd/\eps) = \eps/32$ independently for each vertex in $\tV$. It therefore follows from the Chernoff bound that the number of edges in
$\MM^{\tilde{\pi}}(\tG) \cap \tilde F$ is not bounded by $\eps |\tV|/16$ with probability at most
$\exp(-\eps|\tV|/32)$, which is less than $1/20$ if $|\tV| > 100/\eps$, and we can assume that this is the case. (To circumvent the case of $|\tV| \le 100/\eps$, we can modify the algorithm as follows.
If a sampled vertex belongs to a connected component in $\bV$ of size at most $100/\eps$,
then we can read its connected component in $\tG$ and deterministically find a maximal matching that uses only edges in $\bE$ and self-loops in $\tE$. This all takes at most $O(\bd/\eps^2)$ time, which as we see later, we are allowed to spend per each sampled vertex.)
Therefore, we have
$$|\VC^{\tilde{\pi}}(\tG) \cap \bV| 
    \le 2 |\VCopt(\bG)| + \eps|\bV|/4,$$
with probability at least $1 - 1 / 20$.

Observe that given query access to $G$, we can efficiently provide query access to $\tG$.
Degrees of vertices in $\bV$ are the same as in $G$. For associated vertices
in $\tV$ it is easy to compute their degree in $O(1)$ time, using the degree
of the corresponding vertex in $\bV$. To answer neighbor queries for vertices $v$ in $\bV$,
except for the fixed connections to $v'$, it suffices to notice that if the corresponding edge in $G$ is connected to a vertex in $L$, this connection is replaced by a connection to an appropriate vertex $v''_{i}$. Otherwise, the edge remains in $\bE$. For vertices $v''_{i}$ some number of connections can either be a connection to the corresponding $v$ or a self-loop. This can be checked in $O(1)$ time with a single query to the neighborhood list of $v$. All the other edges are fixed. Therefore, we can simulate an execution of the vertex-cover and the maximal-matching oracles on $\tG$.
Answering every query to $\tG$ requires $O(1)$ time and $O(1)$ queries to $G$.
Sampling vertices uniformly at random from in $\bV \cup \tV$ is more involved, but in our algorithm, we only need to sample vertices from $V$, which we assume we can do.

The expected number of recursive calls to the maximal matching oracle is bounded by $O(\bd/eps^2)$ for a random vertex $v \in \bV \cup \tV$, because the maximum degree and the minimum degree are within a factor of $O(1/\eps)$ and the maximum degree is bounded by $O(\bd/\eps)$. Note that since $3|\bV| \ge |\tV|$, this expectation for a random 
vertex $v \in V$ is at most twice as much, i.e., it is still $O(\bd/\eps^2)$.

For any ranking $\tilde \pi$ of edges in $\tG$,
if we sample $O(1/\eps^2)$ vertices from $V$ with replacement, then the fraction of those for which the oracle answers {\bf TRUE} is within an additive $\eps / 8$ of 
the total fraction of vertices for which the oracle answers {\bf TRUE}.
with probability $1 - 1/20$. Let $\mu$ be the fraction of sampled vertices. We have 
$$|\VCopt(G)| - \eps n/8 \le \mu \cdot n \le 2 |\VCopt(G)| + \eps n/4 + \eps n/8 + \eps n/8$$
with probability $1-1/10$.
Then $(\mu + \eps/8) n$ is the desired $(2,\eps n)$-estimate.
The expected number of calls to the vertex cover and maximal matching oracles is bounded by $O(d/\eps^4)$. As before, without loss of generality, this quantity can be bounded by $O(n^5)$,
which fits into a constant number of machine words. By applying now Lemma \ref{lem:running_time},
we obtain an implementation of the algorithm. 
It runs in $O(d/\eps^3 \cdot \log^3(d/\eps))$ time and makes $O(d/\eps^3 \cdot \log^2(d/\eps))$ queries. Moreover, the probability that the implementation diverges from the ideal algorithm is bounded by $1/5$. Therefore, the implementation outputs a $(2,\eps n)$-estimate with probability 
at least $1-1/5 - 1/10 \ge 2/3$.



\begin{corollary}
There is an algorithm in the adjacency list model that runs in $O(\frac{\tilde d}{\eps^4} \cdot \log^3\frac{\tilde d}{\eps})$ time, makes $O(\frac{\tilde d}{\eps^4} \cdot \log^2\frac{\tilde d}{\eps})$ queries, and with probability $2/3$, outputs a  $(2,\eps n)$-estimate to the minimum vertex cover size.
\end{corollary}


